Pruning Edges and Gradients to Learn Hypergraphs from Larger Sets

This paper aims for set-to-hypergraph prediction, where the goal is to infer the set of relations for a given set of entities. This is a common abstraction for applications in particle physics, biological systems, and combinatorial optimization. We address two common scaling problems encountered in set-to-hypergraph tasks that limit the size of the input set: the exponentially growing number of hyperedges and the run-time complexity, both leading to higher memory requirements. We make three contributions. First, we propose to predict and supervise the \emph{positive} edges only, which changes the asymptotic memory scaling from exponential to linear. Second, we introduce a training method that encourages iterative refinement of the predicted hypergraph, which allows us to skip iterations in the backward pass for improved efficiency and constant memory usage. Third, we combine both contributions in a single set-to-hypergraph model that enables us to address problems with larger input set sizes. We provide ablations for our main technical contributions and show that our model outperforms prior state-of-the-art, especially for larger sets.

==> floats/BPTTwS_performance_comparison.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lccccc}
        \toprule
        &$T_{\text{total}}$&$N_{\text{BPTT}}$&$T_{\text{BPTT}}$&F1&Training time\\
        \midrule
        Truncated BPTT          &   $16$&   $4$ &   $4$ &   $0.84$  &   $3.26\times$\\
                                &   $32$&   $8$ &   $4$ &   $0.89$  &   $6.10\times$\\
        BPTT with fixed skips   &   $16$&   $2$ &   $4$ &   $0.82$  &   $2.08\times$\\
        \emph{(Ours)}           &   $32$&   $4$ &   $4$ &   $0.88$  &   $3.92\times$\\
        BPTT with random skips  &   $16$&   $2$ &   $4$ &   $0.84$  &   $2.08\times$\\
        \emph{(Ours)}           &   $32$&   $4$ &   $4$ &   $0.89$  &   $3.92\times$\\
        \midrule
        BPTT                  &   $4$ &   $1$ &   $4$ &   $0.68$  &   $1.00\times$\\
                              &   $16$&   $1$ &   $16$&   $0.86$  &   $2.52\times$\\
                              &   $32$&   $1$ &   $32$&   $0.82$*  &   $5.12\times$\\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation on BPTT with skips} 
    Compared to BPTT, both TBPTT and BPTTwS can successfully learn $T_{\text{total}}{>}4$ with constant memory cost ($T_{\text{BPTT}}=4$).
    Skipping iterations in the backward passes improves the training time at no test-time performance cost, compared to Truncated BPTT.
    Though BPTT offers poor asymptotic scaling, it remains tractable on small set sizes (in this case $n{=}30$).
    *BPTT with $T_{\text{total}}{=}32$ suffers from training instability stemming from increasing gradient norms over the course of training.
    \cs{Table is not clear, what is our? Order is weird. Order by training time? Why is truncated our opponent? regular BPTT has better efficiency/accuracy trade-off.}}
    \label{tab:BPTTwS performance comparison}
\end{table}

==> floats/hypergraph_refiner.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/hypergraph_refiner.pdf}
  \caption{\textbf{Recurrently predicting hypergraphs.} The input set and an initial guess on the edges are combined into a hypergraph. A recurrent network holistically refines the hypergraph into the prediction. During training, we skip some iterations in the backward pass to improve efficiency and scale to a large number of iterations at constant memory cost. }
    \label{fig:iterative hypergraph refiner}
\end{figure}

==> floats/particle_partitioning.tex <==
\begin{table}
  \caption{\textbf{Particle partitioning results} on three types of jets measured in F1 score and adjusted rand index (ARI). Our method outperforms the baselines on bottom and charm jets, while being competitive on light jets.}
  \label{tab:particles}
  \centering
\resizebox{\columnwidth}{!}{%
  \begin{tabular}{lccccccccc}
    \toprule
    &\multicolumn{3}{c}{\textbf{bottom jets}}&\multicolumn{3}{c}{\textbf{charm jets}}&\multicolumn{3}{c}{\textbf{light jets}} \\
    \cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10}
    Model           & F1 & RI & ARI & F1 & RI & ARI & F1 & RI & ARI\\
    \midrule
    Set2Graph %\citep{serviansky2020set2graph}
    &$0.646\spm{0.003}$&$0.736\spm{0.004}$&$0.491\spm{0.006}$
    &$0.747\spm{0.001}$&$0.727\spm{0.003}$&$0.457\spm{0.004}$
    &$0.972\spm{0.001}$&$0.970\spm{0.001}$&$0.931\spm{0.003}$\\
    Set Transformer
    &$0.630\spm{0.004}$&$0.734\spm{0.004}$&$0.464\spm{0.007}$
    &$0.747\spm{0.003}$&$0.734\spm{0.004}$&$0.466\spm{0.007}$
    &$0.970\spm{0.001}$&$0.967\spm{0.002}$&$0.922\spm{0.003}$\\
    Slot Attention
    &$0.600\spm{0.012}$&$0.703\spm{0.013}$&$0.411\spm{0.021}$
    &$0.728\spm{0.008}$&$0.714\spm{0.009}$&$0.429\spm{0.016}$
    &$0.963\spm{0.002}$&$0.958\spm{0.003}$&$0.895\spm{0.009}$\\
    Ours            
    &$0.679\spm{0.002}$&$0.781\spm{0.002}$&$0.548\spm{0.003}$
    &$0.763\spm{0.001}$&$0.751\spm{0.001}$&$0.499\spm{0.002}$
    &$0.972\spm{0.001}$&$0.969\spm{0.001}$&$0.926\spm{0.002}$\\
    \bottomrule
  \end{tabular}%
}
\end{table}

==> floats/training_algorithm.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
% \begin{minipage}{0.45\textwidth}
\small
\begin{algorithm}[H]
\label{alg:TBPTT}
\SetKwProg{With}{with}{:}{}
\SetKw{KwTo}{in}\SetKwFor{For}{for}{\string:}{}%
\SetKwFunction{Range}{range}%%
\SetKwFunction{Zip}{zip}
\SetKwFunction{NoGrad}{no\_grad}
\SetKwFunction{Initialize}{initialize}
\SetKwFunction{SampleIntegerPartition}{sample}
\SetKwFunction{Refine}{refine}
\SetKwFunction{Loss}{loss}
\SetKwFunction{BP}{backward}
\SetKwFunction{Step}{gradient\_step\_and\_reset}
\SetKwFunction{Reset}{reset\_gradient}
\AlgoDontDisplayBlockMarkers\SetAlgoNoEnd\SetAlgoNoLine%
\SetAlgoLined\DontPrintSemicolon
%\KwResult{Write here the result }
 \KwIn{$\VRT_{\text{input}}, \INC_{\text{target}}, T_{\text{total}}, T_{\text{BPTT}}, N_{\text{BPTT}}$}
 $\HG\coloneqq(\VRT,\EDG,\INC)\leftarrow$ \Initialize{$\VRT_{\text{input}}$}\;
 $T_{\text{skip}}\leftarrow$ \SampleIntegerPartition{$T_{\text{total}}, T_{\text{BPTT}}, N_{\text{BPTT}}$}\;
 \For{$t$ \KwTo $T_{\text{skip}}$}{
  \With{\NoGrad{}}{
    \For{$i$ \KwTo \Range{$t$}}{
     $\HG \leftarrow$\Refine{$\HG$}
    }
  }
  $\mathcal{L}\leftarrow 0$\;
  \For{$i$ \KwTo \Range{$T_{\text{bp}}$}}{
  $\HG \leftarrow$\Refine{$\HG$}\;
  $\mathcal{L}\leftarrow\mathcal{L}$ + \Loss{$\HG,\INC_{\text{target}}$}\;
  }
  \BP{$\mathcal{L}$}\;
  \Step{}\;
 }
 \caption{
 BPTT with skips
%  Inputs are a mini-batch of training examples $\left(\VRT_{\text{input}}, \INC_{\text{target}}\right)$, an integer $T_{\text{total}}$ specifying the total number iterations, an integer $T_{\text{BPTT}}$ specifying the number of iterations to run BPTT on and an integer $N_{\text{BPTT}}$ specifying the number of gradient updates per mini-batch. The function \protect\SampleIntegerPartition{$a,b$} returns a random integer partition of $a$ into $b$ parts.
 }
\end{algorithm}
% \end{minipage}
\end{wrapfigure}

==> sections/experimental_details.tex <==
% adjacency vs incidence
% Building on the idea of solely predicting the set of positive edges, we construct two additional baselines that map from the set of vertices to the set of edges, followed by an incidence indicator network similar to Equation~\ref{eq:incidence}.
% Both Set Transformer and Slot Attention were not designed for set-to-hypergraph tasks, but we consider them as general set-to-set models.
% particle
Set2Graph incurs a prohibitively large memory cost when predicting edges with high connectivity and instead resorts to only predicting edges with at most $2$ connecting vertices, followed by an additional heuristic to infer the partitions.
The input sets consist of 2 to 14 particles, with each particle represented by 10 features.
The target partitionings indicate the common progenitors and restrict the valid incidence matrices to those with a single incident edge per vertex.
We train our method with $T_{\text{total}}{=}16$, $T_{\text{BPTT}}{=}4$, $N_{\text{BPTT}}{=}2$ and a maximum of $10$ edges.
Since each particle can only be part of a single partition, we choose the one with the highest incidence probability at test time.
All models additionally minimize a soft F1 score \citep{serviansky2020set2graph}.
We refer to \citet{shlomi2020graph} for more background information on the task.
Coupled with the performance of the set-to-set based baselines, the results highlight that it is indeed feasible to train without explicitly supervising negative edges.
Furthermore, the relative improvement of our approach compared to the set-to-set baselines hints at the benefits of a holistic refining approach.

% convex hull finding
On convex hull finding in $3$D, we compare our method to the same baselines as in the previous experiment. 
Set2Graph \citep{serviansky2020set2graph} learns to map the set of $3$D points to the $3$rd order adjacency tensor. 
Since storing this tensor in memory is not feasible, they instead concentrate on a local version of the problem, which only considers the $k$-nearest neighbors for each point \citep{serviansky2020set2graph}. 
We train our method with $T_{\text{total}}{=}48$, $T_{\text{BPTT}}{=}4$, $N_{\text{BPTT}}{=}6$ and set $k$ equal to the highest number of triangles in the training data. 
At test time, a prediction admits an edge $e_i$ if its existence indicator $\sigma_i>0.5$. 
Each edge is incident to the three vertices with the highest incidence probability.

% delaunay triangulation
The problem of Delaunay triangulation is, similar to convex hull finding, a well-studied problem in computational geometry and has exact solutions in $\mathcal{O}(n\log{(n)})$ \citep{rebay1993efficient}.
Note that this differs from finding the set of triangles, as an edge no longer remembers which triangles it is part of.

The goal in this task is to predict the adjacency matrix of an ordinary graph -- a graph consisting of edges that connect two vertices -- where the number of edges are greater than the number of vertices.
One could recover the adjacency matrix based on the matrix product of $\INC^T\INC$, by clipping all values above 1 back to 1 and setting the diagonal to 0.
This detour through the incidence matrix is clearly unfavorable, as in this case the incidence matrix actually takes up more compute than the adjacency matrix.
Instead of applying our method directly, we consider a simple adaptation of our approach to the graph setting.
We replace the initial set of edges with the (smaller) set of vertices and apply the same vertex refinements (Equation~\ref{eq:vertex}) on both sets.
This change results in $\EDG{=}\VRT$ for the prediction and effectively reduces the incidence matrix to an adjacency matrix, since it is computed based on all pairwise combinations of $\EDG$ and $\VRT$.
We further replace the concatenation in $\phi_{\INC}$ (Equation~\ref{eq:incidence}) with a sum, to ensure that the predicted adjacency matrix is symmetric and represents an undirected graph.
Two of the main design choices of our approach remain in this adaptation: Iterative refining of the complete graph with a recurrent neural network and BPTT with gradient skips. We train our model with $T_{\text{total}}{=}32$, $T_{\text{BPTT}}{=}4$ and $N_{\text{BPTT}}{=}4$.
At test-time, an edge between two vertices exists if the adjacency value is greater than $0.5$.

% complexity
The number of refinement steps scales sub-linearly with the set size, different from the intrinsic time complexity.
This highlights the property that our approach does not operate incrementally, but instead parallelizes the edge finding process.
Notably, increasing the number of iterations does not introduce any additional parameters, as opposed to increasing the depth or width.
An analogy can be made with an exact algorithm that incrementally constructs the convex hull, but is allocated insufficient computing time, in which case the result will have (more) errors.
By replacing BPTT with truncated BPTT or BPTT with skips, our approach offers a scalable solution for settings with a fixed memory budget

%recurrent vs stacked
For the stacked version, we only compute the loss at the final refinement step, as we observed that supervising all intermediate steps leads to worse performance.
Both versions are trained using normal backprop.
% The results indicate that recurrence constitutes a useful inductive bias on an intrinsically complex problem, especially when supervised over multiple steps.

%-------------------------------------------------------------------
\subsection{Can we actually \emph{learn} tasks that encompass higher-order edges?}
%-------------------------------------------------------------------
% The asymptotic scaling behavior of our approach suggests that it is computationally feasible to address problems with higher-order edges. This advantage is only useful if our method can actually learn the task, which we aim to asses next.
The particle partitioning experiment exemplifies a case where a single edge can connect up to $14$ vertices. Set2Graph \citep{serviansky2020set2graph} demonstrates that in this specific case it is possible to approximate the hypergraph with a graph. They leverage the fact that any vertex is incident to exactly one edge and apply a post-processing step that constructs the edges from noisy cliques. Instead, we consider a task for which no straightforward graph based approximation exists. Specifically, we consider convex hull finding in $10$-dimensional space for $13$ standard normal distributed points.
We train with $T_{\text{total}}{=}32$, $N_{\text{BPTT}}{=}4$ and $T_{\text{BPTT}}{=}4$. The test performance reaches an F1 score of $0.75$, clearly demonstrating that the model managed to learn. This result demonstrates the improved scaling behavior can be leveraged for tasks that are computationally out of reach for adjacency-based approaches.


%backprop with skips
We constrict both truncated BPTT and BPTT with skips to a fixed memory budget, by limiting any backward pass to the most recent $T_{\text{BPTT}}{=}4$ iterations, for $T_{\text{total}}{\in}\{16,32\}$.

This suggests that supervising all iterations, like in TBPTT, is highly redundant and skipping iterations in the weight update phase constitutes an effective approach to reducing said redundancy.
For our method, we observe that sampling random subsequences is more stable than picking fixed time steps.

The results on standard backprop appear to indicate that performance worsens when increasing the number of iterations from $16$ to $32$.
We observe that applying backprop on many iterations leads to increasing gradient norms in the course of training, complicating the training process.
The memory limited versions did not exhibit a similar behavior, evident from the improved performance, when increasing the iterations from $16$ to $32$.

==> sections/method.tex <==
%The general idea of our approach consists of reaching a prediction by iteratively refining an initial guess.
%We start out by combining the input set with a random set of edges into a hypergraph, followed by iterative refinements that update the initial hypergraph in the direction of the solution.
%We illustrate this in Figure~\ref{fig:iterative hypergraph refiner}.
%The refinement steps are instantiated as a recurrent hypergraph neural network that holistically transforms the hypergraph in each step. 
\input{floats/hypergraph_refiner}

% In this section, we present an efficient set-to-hypergraph framework that addresses both the potential pitfalls discussed in the previous section.
% First, we describe how the problem can be modeled as a hypergraph for which the nodes are given but the edges are unknown.
% We assume the number of edges is small, relative to the number of potential candidates, which is the case in many applications as we show in the experiments.
% Next, we present the Recurrent Hypergraph Refiner (RHR) module that takes an initial hypergraph as input and refines it iteratively.
% We leverage the parameter-efficiency from the recurrence to further propose a backpropagation with gradient skips algorithm to address complex problems that require more compute without needing more parameters.

% For a given input set $\mX$, the goal is to produce the corresponding hypergraph.
\subsection{Recurrent Hypergraph Refiner}
The Recurrent Hypergraph Refiner (RHR) maps from an input set $\mX$ of size $n$ to a hypergraph $\HG^{(T)}$, by iteratively refining an initial version $\HG^{(0)}$ for $T$ steps (\autoref{fig:iterative hypergraph refiner}).
In the rest of the section, we first describe each part in $\HG^{(0)}$ and the corresponding initialization.
Next, we present the exact refinement step and explain how the permutation symmetry is maintained.
% Conceptually, we can treat $\mX$ as the nodes of this hypergraph, thus the aim is to infer the edges and their connectivity.

\paragraph{Nodes.}
We construct the initial hypergraph $\HG^{(0)}$ as a tuple that includes the set of nodes $\VRT^{(0)}$, the set of (hyper)edges $\EDG$ and the incidence matrix $\INC$.
The nodes are represented by $d_{\VRT}$-dimensional vectors, each initialized as an affine transformation of an input element: $v_i^{(0)}=Wx_i+b$, where $W$, $b$ are learnable parameters.
This directly assigns each input element an identity as a node in the hypergraph.
Furthermore, the transformation allows for arbitrary hidden dimensions $d_{\VRT}$ that are independent of the input feature dimensions.

\paragraph{Edges.}
Since our goal is to produce the unknown edges and their connections, we sample the edge representations as $e_i\sim\mathcal{N}(\mu, \text{diag}(\sigma))$, with shared learnable parameters $\mu\in\mathbb{R}^d_{\EDG}$ and $\sigma\in\mathbb{R}^d_{\EDG}$.
It is important that the edge representations are initialized i.i.d. so that they are symmetric and different with high probability.
The latter is important for the subsequent permutation equivariant refinements to predict different edges, because any permutation equivariant operation will map both elements to the same output vector.
In practice, this property can already become a problem when edges are sufficiently similar, though we observe it is unnecessary to explicitly lower bound the variance for our chosen architecture.
In many cases, the number of edges in the hypergraph will be small in comparison to all possible ones.
We leverage this key observation and prune all unnecessary edges, by assuming a 

\paragraph{Incidence matrix.}
Similar to the edges, we start out with an empty incidence matrix $\INC=0$ that makes no assumption on the structure.
We design methods to handle the additional complications from this.

\paragraph{Refinement step.}
Each refinement step updates 
% At the beginning, we assume no edges and consequently initialize the incidence matrix as $\INC=0$.

% Each node $v_i\in\VRT$ corresponds to the latent representation of the input element $\vx\in\mX$.


% Notably, our definition does not specify an edge as a subset of vertices.
% Instead, the relational structure of the hypergraph is solely expressed by $\INC$.



\textbf{Definition.} An undirected hypergraph $\HG$ is a $3$-tuple $\HG{=}(\VRT,\EDG,\INC)$, where $\VRT{=}\{v_1,\dots,v_{n}\}$ is the set of vertices, $\EDG{=}\{e_1,\dots,e_{k}\}$ is the set of (hyper)edges and $\INC\in\{0,1\}^{k \times n}$ is the incidence matrix.
We represent vertices and edges as $d_{\VRT}$-dimensional and $d_{\EDG}$-dimensional vectors.
Each entry $\INC_{i,j}$ in the incidence matrix indicates if an edge $e_i$ is incident to vertex $v_j$.
Notably, in our definition an edge is not defined as a subset of vertices.
Instead, the relational structure of the hypergraph is solely expressed by $\INC$.
We assume the number of edges is small, relative to the number of potential candidates, which is the case in many applications as we show in the experiments.
During training, we leverage this property by setting $k$ equal to the maximum number of edges for any training example and effectively reduce the memory requirement of $\INC$ to a tractable size.
Furthermore, we relax the constraint on $\INC_{i,j}\in\{0,1\}$ to continuous values $\INC_{i,j}\in[0,1]$, in order to facilitate the usage of standard neural networks for modelling the incidence structure.
The continuous incidence matrix instead indicates the probability that $e_i$ and $v_j$ are incident.

\textbf{Initialization.} $\VRT$ is initialized from a learned affine transformation of the set of input entities.
Each element in $\EDG$ is sampled i.i.d. from an isotropic normal distribution with learned parameters.
For $\INC$, we do not assume the existence of any connections at the beginning and correspondingly initialize it to $0$.
It is important that the elements in $\EDG$ are independently sampled from a distribution with sufficient variance. 
For any two edges in $\EDG$ with identical feature vectors, any permutation equivariant neural network will map both elements to the same output vector.
In practice, this property can already become a problem when edges are sufficiently similar.
We observe it is unnecessary to explicitly lower bound the variance for our chosen architecture.
We denote the initial hypergraph as $\HG^{(0)}$.

\textbf{Refinement step.} The refinement function $\phi$ performs a holistic update $\phi(\HG^{(t-1)}){=}\HG^{(t)}$ at each iteration $t$.
We instantiate $\phi$ as three different neural networks $\phi_{\VRT}, \phi_{\EDG}, \phi_{\INC}$, each responsible for updating the vertices, edges and the incidence matrix, respectively.
Each entry $\INC_{i,j}$ in the incidence matrix is updated independently at each iteration $t$, based on the $j$-th vertex, the $i$-th edge and the incidence from the previous step $t-1$:
\begin{equation} \label{eq:incidence}
    \INC^{(t)}_{i,j}=\phi_{\INC}\left(v^{(t-1)}_j, e^{(t-1)}_i, \INC^{(t-1)}_{i,j}\right),
\end{equation}
where we instantiate $\phi_{\INC}$ as a multilayer perceptron in our experiments.
The vertices and edges are further refined based on the updated relational structure:
\begin{align}
    \VRT^{(t)} &= \phi_{\VRT}\left(\left\{\left[v_j^{(t-1)}, \rho_{\EDG\rightarrow\VRT}\left(j,t\right), v_j^{(0)}\right] \middle| j=1\dots n\right\}\right)
    &
    \rho_{\EDG\rightarrow\VRT}\left(j,t\right) &= \sum_{i=1}^{k} \INC_{i,j}^{(t)} e_i^{(t-1)}
    \label{eq:vertex}\\
    \EDG^{(t)} &= \phi_{\EDG}\left(\left\{\left[e_i^{(t-1)}, \rho_{\VRT\rightarrow\EDG}\left(i,t\right)\right] \middle| i=1\dots k\right\}\right)
    &
    \rho_{\VRT\rightarrow\EDG}\left(i,t\right) &= \sum_{j=1}^{n} \INC_{i,j}^{(t)} v_j^{(t-1)}
    \label{eq:edge}
\end{align}
where $[\cdot]$ denotes the concatenation and $\phi_{\VRT}, \phi_{\EDG}$ are permutation equivariant neural networks, which we instantiate as DeepSets \citep{zaheer2017deep} in the experiments.
The aggregation functions $\rho_{\EDG\rightarrow\VRT}, \rho_{\VRT\rightarrow\EDG}$ sum over all edges and vertices, weighted by their respective incidence probability at time $t$.
We add skip-connections to $\phi_{\VRT}$ and $\phi_{\EDG}$ for $\VRT^{(t-1)}$ and $\EDG^{(t-1)}$, to facilitate training large number of iterations \citep{he2016deep}.
Additionally, we apply layer normalization \citep{ba2016layer} to both the input and output (following the skip connection) of $\phi_{\VRT}$ and $\phi_{\EDG}$.
Previous works observed both the skip-connections and layer normalization to help speed up the training convergence in the context of a recurrent neural network \citep{locatello2020object}.
While the concatenation facilitates cross-communication between vertices and edges, the set neural network directly supplies context from the other vertices and edges, avoiding a detour through the incidence structure.

\textbf{Variable number of edges.}
Different hypergraph instances may admit differing number of edges.
We set $k$ equal to the cardinality of the largest set of edges amongst all training examples and pad the target incidence matrix with additional rows of $0$, resulting in an incidence matrix of shape $k\times n$ for all examples.
An edge that is incident to no vertex, i.e., $\INC_k{=}0$, can be interpreted as non-existent.
Usually the values of the predicted incidence matrix will not be exactly $0$ or $1$, requiring an additional decision procedure to determine if an edge exists and which vertices it connects to.
A simple approach is to decide the incidence structure locally for each entry in the incidence matrix.
This approach ignores fixed structures that are inherent in many problems, e.g., each edge connects exactly $3$ (or no) vertices in a convex hull of $3$-dimensional point sets.
To improve the naive local version, while keeping the decision process simple, we add an existence indicator $\sigma_i^{(t)}$ that is computed as a dot product between the edge $e_i^{(t)}$ and a learned weight vector, followed by a sigmoid function.
Using the existence indicator, we update the incidence matrix:
\begin{equation} \label{eq:existence}
    \hat{\INC}^{(t)}_i = \sigma_i^{(t)}\INC^{(t)}_i,
\end{equation}
which replaces the incidence information used for aggregation in $\rho_{\EDG\rightarrow\VRT}$ and $\rho_{\VRT\rightarrow\EDG}$.
With an explicit existence indicator we can simply choose the $3$ vertices with the highest incidence probability for each existing edge in the $3$D convex hull example.

\textbf{Iterative refinement.}
The prediction at test-time is attained after applying the refinement step, described in \Crefrange{eq:incidence}{eq:existence}, for $T_{\text{total}}$ number of times.
Our approach can be considered an instance of a recurrent neural network (RNN), as each refinement step uses the same set of parameters at each iteration $t$.
Different from conventional RNNs, we structure the latent state of our network as a hypergraph and inject the same input at every time step.
Intuitively, the recurrent architecture provides the neural network with multiple processing steps to consider the global context $\INC$, in the prediction of the local structures $\INC_{i,j}$.
In contrast to auto-regressive approaches, we consider all $\INC_{i,j}$ simultaneously.
Thereby, we do not impose any artificial order on the edges and facilitate parallelization in the problem-solving procedure.
% Different hypergraph prediction problems may vary in their level of difficulty, potentially necessitating many refinement steps.
% Ideally, one should be able to specify an arbitrary number of total refinement steps, accounting for resource limitations and performance requirements.

\textbf{BPTT with gradient skips.}
The common learning method for RNNs is backpropagation through time (BPTT) \citep{pearlmutter1995gradient, robinson1987utility, werbos1988generalization, mozer1989focused}. Conceptually BPTT treats the forward process as a feedforward neural network with weight-tied parameters and applies backpropagation to update the network parameters with respect to the gradients of a loss function.
Applying BPTT on the entire sequence of $T_{\text{total}}$ refinement steps is prohibitive for large $T_{\text{total}}$, due to memory costs growing in $\mathcal{O}(T_{\text{total}})$.
Instead, we approximate the complete gradient by applying BPTT on selected subsequences of length $T_{\text{BPTT}}$, with skips in between different subsequences.
By limiting the length of the backward pass in this way, our memory usage remains constant over time.
We select subsequences such that there are zero or more iterations in between any pair of subsequences.
In the case when there are exactly $0$ iterations in between any consecutive subsequences, we recover truncated BPTT \citep{williams1990efficient}, which in its more general form also permits overlaps in the iterations. 
%
%Figure \ref{fig:SBPTT} illustrates the differences between BPTT, truncated BPTT and our training algorithm.
%
% In order to justify omitting some iterations during all backward passes, we liken our recurrent network to an iterative optimization algorithm.
% For $T_{\text{BPTT}}{=}1$, our training algorithm learns a $\phi$ by minimizing the loss $\mathcal{L}(\phi(\HG^{(t-1)}), \INC_{\text{target}})$ at every time step $t$.
% Notably, the hypergraph $\HG^{(t-1)}$ constitutes the only time-dependent part of the loss term.
% Alternatively, one may independently sample $\HG^{(t-1)}$ at every time step $t$ from some fixed distribution.
% Optimally, this would result in a $\phi$ that reduces the loss between any hypergraph and the target for some given set of vertices.
% Skipping step $t{=}0$ in this case has no impact on training, since a similar hypergraph may appear at any later time step.
% In practice, it is more efficient to train $\phi$ on the trajectory between $\HG^{(0)}$ and $\HG^{(T_{\text{total}})}$, instead of random samples.
% Though similar to the case with randomly sampled hypergraphs, it is unnecessary to supervise each individual iteration.
We liken our recurrent network to an iterative optimization algorithm, that is learned by optimizing $\mathcal{L}(\phi(\HG^{(t-1)}), \INC_{\text{target}})$ at all time steps $t$.
Supervising all iterations is redundant, when the hypergraphs are similar at different steps, motivating us to skip some iterations in the backward passes to reduce the training time.

\input{floats/training_algorithm}
Algorithm \ref{alg:TBPTT} describes the training procedure in pseudocode, leaning on the PyTorch (BSD) syntax \citep{NEURIPS2019_9015}.
For each mini-batch, we sample a list of integers $T_{\text{skip}}$, that determine the number of skipped steps, i.e., refinement calls that are not part of any backward pass.
The total number of skipped steps is $T_{\text{total}}{-}T_{\text{BPTT}}{\cdot}N_{\text{total}}$, where $N_{\text{total}}$ denotes the number of gradient updates per mini-batch. 
We consider two alternative distributions for $T_{\text{skip}}$: 1. Evenly distribute the skipped steps, or 2. Randomly partition the number of skipped steps into $N_{\text{total}}$ parts (with $0$'s).
This training scheme can be interpreted as adapting the refiner to work on different initial hypergraphs, with a random one at the beginning and arbitrarily well refined ones later on.

%CS can go to supplemental
%\input{floats/BPTTwS_comparison}

\textbf{Training objective.}
During training, we minimize the element-wise binary cross entropy of the target and predicted incidence matrix. While the column (vertices) order is given by the input, the rows (edges) may be in arbitrary order due to independent and identically distributed random initialization. We match the edges between the target and the prediction with Hungarian matching \citep{kuhn1955hungarian}. We apply the loss on each intermediate incidence matrix ${\INC}^{(t)}$ to encourage iterative improvements.

\textbf{Computational complexity.}
The space complexity of $\HG$ is in $\mathcal{O}(nk)$, offering an efficient representation for hypergraphs when the maximal number of edges $k$ is relatively low.
Problems that involve edges connecting many vertices benefit from this choice of representation, as the space requirement does not scale with the maximal connectivity of an edge.
During training, BPTT further scales the memory requirement by a factor of $T_\text{BPTT}$, possibly limiting the number of refinement steps.
Our proposed training algorithm does not directly scale with $T_\text{total}$, offering a tractable solution for problems requiring many iterations.
The loss computation is dominated by the Hungarian matching, requiring time in $\mathcal{O}(k^3)$.
This computational cost is further scaled by the factors $N_\text{BPTT}$, $T_\text{BPTT}$ and the mini-batch size.
In practice, the impact from $T_\text{BPTT}$ and the mini-batch size are dampened by applying the matching algorithm in parallel.
In contrast to that, each gradient update step happens sequentially, motivating smaller choices for $N_\text{BPTT}$, to reduce the training time.
By randomly skipping refinement steps during training, we require less gradient update steps for fixed $T_\text{BPTT}$ and $T_\text{total}$, resulting in faster training.
